Wholesale Market Participation of DERA: DSO-DERA-ISO Coordination

Distributed energy resource aggregators (DERAs) must share the distribution network together with the distribution utility in order to participate in the wholesale electricity markets that are operated by independent system operators (ISOs). We propose a forward auction that a distribution system operator (DSO) can utilize to allocate distribution network access limits to DERAs. As long as the DERAs operate within their acquired limits, these limits define operating envelopes that guarantee distribution network security, thus defining a mechanism that requires no real-time intervention from the DSOs for DERAs to participate in the wholesale markets. Our auctions take the form of robust and risk-sensitive markets with bids/offers from DERAs and utility's operational costs. Properties of the proposed auction, e.g., resulting surpluses of DSO and the DERAs, and the auction prices, along with empirical performance studies, are presented.

==> BoseScribles_v0.tex <==

\section{Bose's scribles}
\newcommand{\CVAR}[2]{\textrm{CVaR}_{#1}\left[ #2 \right]}

{\bf Verify the worst case scenario:}

$A = A_+ - A_-$. Suppose $p \in [\ul{p}, \ol{p}]$. What is the maximum value of $A p$, elementwise? Cong's answer is $A_+ \ol{p} - A_-\ul{p}$. 

We have $A=(1, -1)$, $p \in [-1, 2] \times [-2, 1]$. $A_+ = (1,0)$, $A_- = (0,1)$. $\ol{p} = (2, 1)^T$, $\ul{p} = (-1, -2)^T$.
$A_+ \ol{p} - A_-\ul{p} = 2 - (-2) = 4$

What is the smallest value of $A p$? Cong's answer is $A_+ \ul{p} - A_- \ol{p}$. Calculating this we get, $(1,0).(-1,-2) - (0,1).(2, 1) = -2$. Largest value of $ -A p = A_- \ol{p} - A_+ \ul{p}$. This is indeed 2!

{\bf Derive the CVaR constraint:}

\begin{align}
    \begin{aligned}
        & \CVAR{\delta}{A(p_k + p_0)} \leq \ol{b} \; \forall p_k \in [-\ul{C}_k, \ol{C}_k]
        \\
        &\iff A p_k + \CVAR{\delta}{Ap_0} \leq \ol{b} \; \forall p_k \in [-\ul{C}_k, \ol{C}_k]
        \\
        &\iff A_+ \ol{C}_k + A_- \ul{C}_k  + \CVAR{\delta}{Ap_0} \leq \ol{b}
        \\
        &\iff \CVAR{\delta}{Ap_0} \leq \ol{b} - A_+ \ol{C}_k - A_- \ul{C}_k
        \\
        &\iff \min_{\ol{t}} \ol{t} + \frac{1}{1-\delta}\E\left[ Ap_0 - \ol{t}  \right]^+ \leq \ol{b} - A_+ \ol{C}_k - A_- \ul{C}_k.
    \end{aligned}
\end{align}
Dropping the min as usual, we get the constraint
\begin{align}
    \ol{t} + \frac{1}{1-\delta}\E\left[ Ap_0 - \ol{t}  \right]^+ + A_+ \ol{C}_k + A_- \ul{C}_k \leq \ol{b}.
\end{align}
Scenario-based version will be
\begin{align}
    \ol{t} + \frac{1}{1-\delta}\frac{1}{S}\sum_{s=1}^S\left[ A p_0[s] - \ol{t}  \right]^+ + A_+ \ol{C}_k + A_- \ul{C}_k \leq \ol{b}.
\end{align}

Let us now derive the lower bound.
\begin{align}
    \begin{aligned}
        & \CVAR{\delta}{-A(p_k + p_0)} \leq -\ul{b} \; \forall p_k \in [-\ul{C}_k, \ol{C}_k]
        \\
        &\iff -A p_k + \CVAR{\delta}{-Ap_0} \leq -\ul{b} \; \forall p_k \in [-\ul{C}_k, \ol{C}_k]
        \\
        &\iff A_- \ol{C}_k + A_+ \ul{C}_k + \CVAR{\delta}{-Ap_0} \leq -\ul{b}
        \\
        &\iff \CVAR{\delta}{-Ap_0} \leq -\ul{b} - A_- \ol{C}_k - A_+ \ul{C}_k
        \\
        &\iff \min_{\ul{t}} \ul{t} + \frac{1}{1-\delta}\E\left[ -Ap_0 - \ul{t}  \right]^+ \leq -\ul{b} - A_- \ol{C}_k - A_+ \ul{C}_k.
    \end{aligned}
\end{align}
Dropping the minimum as usual, we get 
\begin{align}
     \ul{t} + \frac{1}{1-\delta}\E\left[ -Ap_0 - \ul{t}  \right]^+ +  A_- \ol{C}_k + A_+ \ul{C}_k\leq -\ul{b}. 
\end{align}
The scenario approximation then becomes 
\begin{align}
     \ul{t} + \frac{1}{1-\delta}\frac{1}{S}\sum_{s=1}^S\left[ -A p_0[s] - \ul{t}  \right]^+ +  A_- \ol{C}_k + A_+ \ul{C}_k\leq -\ul{b}. 
\end{align}


{\bf Understand CVaR:}

For random variable $X$ with a smooth cdf, we have
\begin{align}
    \CVAR{\delta}{X} = \E[X | X \geq F_X^{-1}(\delta)].
\end{align}
In the paper RU2000, they showed that 
\begin{align}
    \CVAR{\delta}{X} = \min_{t} \left\{ t + \frac{1}{1-\delta}\E[X - t]^+ \right\}.
    \label{eq:def.CVAR}
\end{align}

In the paper RU2002, the expected shortfall definition was shown to be difficult when the distribution of $X$ can have atoms. They even introduced this notion of CVaR$_+$ and CVaR$_-$. Then, they proposed to use a variational definition of the risk measure itself, i.e., use \eqref{eq:def.CVAR} as the definition of CVaR. This definition ensures that $\CVAR{\delta}{X}$ varies continuously with $\delta$, a crucially important property of a good risk measure.

Showing the translation property of CVaR. 
\begin{align}
    \CVAR{\delta}{X+a} = \min_{t} \left\{ t + \frac{1}{1-\delta}\E[X + a - t]^+ \right\} 
\end{align}
Let us do a change of variables. Let $t' = t - a$. Then, we have
\begin{align}
    \CVAR{\delta}{X+a} 
    &= \min_{t'} \left\{ t' + a + \frac{1}{1-\delta}\E[X + t']^+ \right\} 
    \\
    &= a + \min_{t'} \left\{ t' + \frac{1}{1-\delta}\E[X + t']^+ \right\} 
    \\
    &=a + \CVAR{\delta}{X}
\end{align}


==> DERA_DSO_v0.tex <==
We consider the interaction model among DSO, RTO/ISO and multiple DERAs shown in Fig. \ref{fig:DERAmodel}, which extends the generic model in \cite{chen22competitive} to the case with multiple DERAs. All DERAs need to use DSO's physical infrastructure to deliver power to  and from its customers to the wholesale market. And this work focuses on market mechanisms for DSO to allocate network resources to DERAs for their wholesale market participations under FERC order 2222.

%  Fig. \ref{fig:DERAmodel} also shows the financial flow, power flow and control signals interacted between DERA and its customers, DERA and RTO/ISO, and DERA and DSO. And DSO need to assign limited physical power injection capacity of the distribution network to multiple DERAs.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.8]{Figs/DERA_DSO.eps}
    \caption{Power flow, financial flow and control interactions in the  DERA-DSO coordination model.}
    \label{fig:DERAmodel}
\end{figure}

In this generic interaction model, profit-seeking DERAs aggregate DERs in a distribution system for wholesale market participation. And each DERA is a single-bill service provider of residential, commercial, and industrial customers. 

As for the injection access allocation of the distribution network, DERAs participate in an auction hosted by DSO to acquire the rights to use the distribution network to deliver aggregated DERs to the transmission system. DSO is responsible to maintain the voltage stability and provide reactive power support in the distribution network.




%---------------



==> Discuss_v0.tex <==
\tcr{limitations of this paper}
We discuss in this section aspects of DSO-DERA  that are not covered in this two-part paper. The purpose is to provide a broader perspective and contexts beyond the scope of this paper.


emergency coordination and override of DSO for scheduling.

==> ICaggregation_v5.tex <==
We now explain the offer formation for the induced benefit functions $\varphi_k$ of DERA $k$. All variables and parameters in this section are associate with DERA $k$, and we omit subscript $k$ for simplicity. DERAs construct their bids for the network access auction by maximizing their profits assuming forecast available renewable. %from offering their aggregated productions to the wholesale market. 


We first extend the DER aggregation approach in \cite{chen22competitive} to the case with injection access constraints for the optimal decision-making of DERA with the aggregated prosumers. With this injection access-constrained optimization, we compute  the optimal bids $\varphi$ from DERA to the forward auction (\ref{eq:auction.2}) allocating network accesses. 
 
\subsection{Profit Maximizing DER Aggregation}
 
We consider the case that DERA maximizes her own surplus, while providing $\zeta>1 $ times those surpluses to the aggregated customers she serves than the utility's rate for distributed generation (DG). This section is an extension of the DER aggregation approach in \cite{chen22competitive} to the case with injection access constraints. Without loss of generality, we assume each bus has one prosumer, thus the DERA aggregating $N$  prosumers will need to have injection/withdrawal accesses for these $N$ buses. DERA receives  payment $\omega^i \in \Rset$ from each prosumer indexed by $i$ and directly buys or sells its aggregated energy in the wholesale market with the locational marginal price $\pi_{\mbox{\tiny LMP}} \in \Rset$. To maximize DERA surplus between the received payment and the payment to the wholesale market,  DERA uses the optimization below. %\footnote{Resources aggregated by DERA $k$ have subscript $k$, which are dropped here for simplicity, eg. $d^i$, $r^i$, $S^i_{{\textrm{NEM}}}$, $U^i$, $V^i$, etc.}.
%\vspace{-0.2cm}
\begin{align}
    \begin{aligned}
    \varphi(\v{\ul{C}},\v{\ol{C}}) =& \underset{\omegabf,\dbf}{\text{maximum}} && 
    % \Pi(\omegabf,\dbf) := 
    \sum_{i=1}^N (\omega^i-\pi_{\mbox{\tiny LMP}} (d^i-r^i)), 
    \\
    & \text{such that}  
    &&\zeta S^i_{{\textrm{NEM}}}(r^i) \le U^i(d^i)-\omega^i,
    \\
    &&&
    \ul{d}^i \le d^i \le  \ol{d}^i,
    \\ 
    &&& 
    \ul{C}^{i} \le   r^i-d^i \le  \ol{C}^{i},
    \\
    &&& i =1,\ldots,N.   
    \end{aligned}
    \label{eq:DERAsurplus_LnGP}
\end{align}
%\vspace{-0.3cm}

The first constraint encodes the  competitive nature of DERA, which  guarantees that the prosumer surplus is at least $\zeta$ times the surplus under the net energy metering (NEM X). Explicit formulation of prosumer surplus $S^i_{{\textrm{NEM}}}(r^i)$ is shown in the appendix. The second constraint is prosumer consumption limits, and the last constraint is injection and  withdrawal access limits. 


\subsection{Benefits of Aggregation and Bid Formation}
The following proposition introduces the optimal closed-form solution of (\ref{eq:DERAsurplus_LnGP}). The optimal DERA surplus is decomposed into three terms, the surplus dependent on the withdraw access $\ul{\varphi}^i({\ul{C}}^i)$, the surplus dependent on the  injection access $\ul{\varphi}^i({\ul{C}}^i)$, and the surplus independent of the network access $h^i-\zeta S^i_{{\textrm{NEM}}}(r^i)$. 
 
\begin{proposition}[Optimal DERA Decision]\label{Prop:DERA}
The optimal solution of \eqref{eq:DERAsurplus_LnGP} is given by%\footnote{Notation $[z]_a^b:=\min\{b,\max\{z, a\}\}$. }
%\vspace{-0.2cm}
\begin{align}
\begin{aligned}
% d^{i\star}(\pi_{\mbox{\tiny LMP}},r^i)
% &=[(V^i)^{-1}(\pi_{\mbox{\tiny LMP}})]_{\max\{\ul{d}^i, r^i-\ol{C}^{i}\}}^{\min\{\ol{d}^i, r^i-\ul{C}^{i}\}},
% \\
d^{i\star}(\pi_{\mbox{\tiny LMP}},r^i)
&=\min\{r^i-\ul{C}^{i}, \max\{\hat{d}^i, r^i-\ol{C}^{i}\}\},
\\
\omega^{i\star}(d^{i\star},r^i)
&= U^i(d^{i\star})-\zeta S^i_{{\textrm{NEM}}}(r^i),
\end{aligned}
\end{align}%\vspace{-0.1cm}
where $\hat{d}^i:=\min\{{\ol{d}}^i,\max\{(V^i)^{-1}(\pi_{\mbox{\tiny LMP}}), {\ul{d}}^i\}\}$.

The optimal DERA surplus is given by
%\vspace{-0.3cm}
\begin{align}\label{eq:bidCurve}
\varphi(\v{\ul{C}},\v{\ol{C}})=&\sum_{i=1}^N\ul{\varphi}^i({\ul{C}}^i)+\sum_{i=1}^N\ol{\varphi}^i({\ol{C}}^i)\\\nn
&+\sum_{i=1}^N (h^i-\zeta S^i_{{\textrm{NEM}}}(r^i)),
\end{align}%\vspace{-0.2cm}

\begin{align*}
\text{where } h^i&:=U^i(\hat{d}^i)-\pi_{\mbox{\tiny LMP}} (\hat{d}^i-r^i),\\
\ul{\varphi}^i({\ul{C}}^i)&:=\begin{cases}
U^i(r^i-\ul{C}^{i})+\pi_{\mbox{\tiny LMP}}\ul{C}^{i}-h^i, & \text{if } r^i\le   q_+^i,\\
0,&\text{otherwise},
% \nn
\end{cases}
\\
\ol{\varphi}^i({\ol{C}}^i)&:=\begin{cases}
U^i(r^i-\ol{C}^{i})+\pi_{\mbox{\tiny LMP}}\ol{C}^{i}- h^i, & \text{if }q_-^i \le r^i,\\
0,& \text{otherwise},
\end{cases}
\\
q_-^i &:=\ol{C}^{i} +\max\{(V^i)^{-1}(\pi_{\mbox{\tiny LMP}}),\ul{d}^i\},
\\
q_+^i &:=\ul{C}^{i}+\min \{(V^i)^{-1}(\pi_{\mbox{\tiny LMP}}),\ol{d}^i\}.
\end{align*}
\end{proposition}
The proof follows the Karush-Kuhn-Tucker optimality conditions for \eqref{eq:DERAsurplus_LnGP} (see appendix \cite{ChenBoseTong22Access} for details). When there's no binding constraints for network access limits, $\hat{d}^i$ is the optimal consumption of prosumer $i$, and $h^i-\zeta S^i_{{\textrm{NEM}}}(r^i)$ is the benefit of DERA from prosumer $i$. When there's binding network access constraints, the optimal consumption $d^{i\star}(\pi_{\mbox{\tiny LMP}},r^i)$ equals to $\hat{d}^i$ truncated by the network access limits, and benefit of DERA is modified by $\ol{\varphi}^i({\ol{C}}^i)$ and $\ul{\varphi}^i({\ul{C}}^i)$. 

We remark that the optimal DERA benefit $\varphi(\v{\ul{C}},\v{\ol{C}})$ is separable across injection and withdrawal access, and across prosumers at different distribution buses. Furthermore, at most one of $\ol{\varphi}^i({\ol{C}}^i)$ and $\ul{\varphi}^i({\ul{C}}^i)$ can be nonzero, depending upon the renewable generation $r^i$ for prosumer $i$. When $r^i\le   q_+^i$, $\ul{\varphi}^i({\ul{C}}^i)$ is nonzero and prosumer at bus $i$ is a consumer with binding network withdrawal access constraints; when $q_-^i \le  r^i $, $\ol{\varphi}^i({\ol{C}}^i)$ is nonzero and prosumer at bus $i$ is a producer with binding network injection access constraints.  
% Therefore, the induced utilities of DERA submitted to DSO can be implied by the supply offers  $\nabla_{\tiny \v{\ul{C}}_k}\ul{\varphi}_k(\v{\ul{C}}_k) =(\frac{d}{d~ {\ul{C}}^i_k}\ul{\varphi}^i_k({\ul{C}}^i_k))$ for the withdrawal access, and $ \nabla_{\tiny  \v{\ol{C}}_k}\ol{\varphi}_k(\v{\ol{C}}_k) =(\frac{d}{d~ {\ol{C}}^i_k}\ol{\varphi}^i_k({\ol{C}}^i_k)) $ for the injection access. 

Therefore, DERA can construct its bids for injection and withdrawal access as  $\ol{\varphi}^i({\ol{C}}^i)$ and $\ul{\varphi}^i({\ul{C}}^i)$ at different buses. In practice, piece-wise linear apprixmations of those bids are needed to be included in the access auction problem (\ref{eq:auction.2}).  %\footnote{Subgradients can be used at the non differentiable points of $\ul{\varphi}_k^{i}, \ol{\varphi}_k^{i}$.}
% \begin{align}
%     {\ul{C}}^i_k=(\ul{\varphi}_k^{i,'})^{-1}(\ul{\lambda}^i), 
%     \
%     {\ol{C}}^i_k=(\ol{\varphi}_k^{i,'})^{-1}(\ol{\lambda}^i),
%     \label{eq:supplyOffer}
% \end{align}
% respectively, from its marginal surplus, within $\ul{C}^{i, \text{\tiny{max}}}_k, \ol{C}^{i, \text{\tiny{max}}}_k$.

% , where 
% Given the locational allocation prices $\ol{\lambda}^i$ and $\ul{\lambda}^i$  for injection and  at bus $i$, the market clearing quantity for the injection access is decided by the supply offer ${\ul{C}}^i_k=(\ul{\varphi}_k^i')^{-1}(\ol{\lambda}^i)$.
 
% The aggregator marginal profit of the bid-in injection access is 

% \begin{align}
%     \frac{\partial \Pi(\omegabf^*,\dbf^*)}{\partial \ol{C}^{i}_k}=\begin{cases}
% -U^i'(r^i-\ol{C}^{i}_k)+\pi_{\mbox{\tiny LMP}}, & \text{if }\ol{C}^{i}_k \le q_+^i,\\
% 0,& \text{otherwise}.
% \end{cases}
% \end{align}

% \begin{align}
%     \frac{\partial \Pi(\omegabf^*,\dbf^*)}{\partial \ul{C}^{i}_k}=\begin{cases}
% -U^i'(r^i-\ul{C}^{i}_k)+\pi_{\mbox{\tiny LMP}}, & \text{if }q_-^i\le\ul{C}^{i}_k,\\
% 0& \text{otherwise}.
% \end{cases}
% \end{align}
% where we denote  $q_+^i:=\min\{r^i-(V^i)^{-1}(\pi_{\mbox{\tiny LMP}}), r^i-\ul{d}^i\}$ and $ q_-^i:=\max \{r^i-(V^i)^{-1}(\pi_{\mbox{\tiny LMP}}), r^i-\ol{d}^i\}$.

% So, the bid-in marginal utility curves submitted to the auction problem (\ref{eq:auction.2}) from DERA $k$ at all buses are


% \begin{align}
% \nabla_{\v{\ol{C}}_k}\ol{\varphi}_k(\v{\ol{C}}_k)=\nabla_{\v{\ol{C}}_k}\Pi^*(\cdot),~\nabla_{\v{\ul{C}}_k}\ul{\varphi}_k(\v{\ul{C}}_k)=\nabla_{\v{\ul{C}}_k}\Pi^*(\cdot).
% \end{align}

% $\Pi^*_k(\v{\ul{C}}_k,\v{\ol{C}}_k)=\varphi_k(\v{\ul{C}}_k,\v{\ol{C}}_k) $.
% $U(\cdot)$ concave, $U'(\cdot)$ non increasing, $\frac{\partial \Pi(\cdot)}{\partial \bar{q}_n}$ non decreasing. $\frac{\partial \Pi(\cdot)}{\partial \underline{q}_n}$ non increasing. $f(\bar{q}_n,\underline{q}_n)$ non increasing.

% $C_n(\cdot)$ non increasing.
% With the bid-in marginal utility curve above, a complete formulation of the bid-in utility function is shown in Sec.~\ref{sec:BidU}.




